A Behavioral Approach to Visual Navigation with Graph Localization Networks

Inspired by research in psychology, we introduce a behavioral approach for visual navigation using topological maps. Our goal is to enable a robot to navigate from one location to another, relying only on its visual input and the topological map of the environment. We propose using graph neural networks for localizing the agent in the map, and decompose the action space into primitive behaviors implemented as convolutional or recurrent neural networks. Using the Gibson simulator, we verify that our approach outperforms relevant baselines and is able to navigate in both seen and unseen environments.

==> sec/intro.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/Pull-4.pdf}
    \caption{Our Turtlebot agent operates in a cluttered indoor environment (left) that is represented as a topological map (middle). Using the depth information (right) along with the topological map, the agent must navigate to its destination, specified as a location within the topological map.}
    \label{fig:pull}
\end{figure*}

\section{Introduction}

% Might remove this paragraph
% Imagine visiting an old friend's house, going to a movie theater that you have not visited in a while, or walking around your office floor. Whether or not objects or furniture have been moved, people have no problem with navigating their way around indoor environments. Even more impressively, given a high-level, natural language description of how to reach a specific destination, humans are able to deduce a precise path through the environment and execute it even in unknown spaces.

Despite the ever-changing state of our indoor environments due to rearrangements in furniture, changes in lighting, or the simple accumulation of clutter, humans are able to seamlessly navigate through these ``dynamic'' spaces as if nothing in the environment has changed at all. Unlike robots, humans are able to easily avoid collisions, and they rarely get lost in familiar spaces. Impressively, this can all be done without any reliance on precise metric information. Instead, prior studies have shown that they rely on coarse spatial layouts in the form of ``cognitive maps'' (\textbf{cite Tolman}).

% Research has suggested that successful navigation is not dependent on geometric accuracy, but rather that asdf. Geometric information can be used for optimizing route planning or resolving topological ambiguities.

Studies in psychology have suggested that at the core of such cognitive maps for large-scale spaces is a topological description (\textbf{cite Kuipers and his [29, 35, 39]}). Research has shown that animals do not rely on metric representations, and instead utilize a navigation strategy that is supported by qualitative topological knowledge of the environment (rephrase) (cite Koltun and his Gillner Mallot, Wang Spelke, and Foo). Geometric information, on the other hand, can rather be used for resolving topological ambiguities or optimizing route planning (\textbf{cite Kuipers}).

% Even without visiting an area, we are still able to (reason about the environmental structure and) build topological maps about unknown environments (semi parametric topological maps, xiaoxue and ashwini). For example, given a natural language description of how to get from A to B, we can successfully deduce the precise path for a given topological map.

\begin{figure}
    \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{fig/top_view.pdf}
    \caption{Caption1}
    \label{fig:stanford-2d-3d-s:top-view}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{fig/3d_mesh.pdf}
    \caption{Caption2}
    \label{fig:stanford-2d-3d-s:3d-mesh}
    \end{subfigure}
    
    \caption{Caption for two-figure image}
    \label{fig:stanford-2d-3d-s}
\end{figure}

\textit{Brief overview of prior work}

However, most approaches to visual navigation today still rely on building metric maps. Classical approaches require precise localization and depend on accurate geometry, making the algorithms brittle, susceptible to changes in the environment, and prone to failure in textureless scenes \cite{gupta2017cognitive,gupta2017unifying,sepulveda2018deep}. For example, these methods do not work well in environments that have been re-arranged (e.g. furniture). Moreover, the algorithms struggle with certain spaces such as textureless environments (e.g. textureless hallways). Classical approaches also struggle to transfer knowledge about prior environments to new environments.

More recently, deep learning approaches to navigation have gained popularity. These approaches are usually either reactive, unstructured memory, navigation-specific memory.

Many of these works rely on ground truth ego-motion (Mirowski, Gupta, Parisotto and Salakhutdinov).

Modern approaches such as [Mirowski, Zhu] have ignored how to represent the space. Gupta et al. also take as input the target location relative to the current position. We act in continuous space and do not allow collisions. Moreover, many RL approaches have been done in unrealistic synthetic environments. However, real-world indoor spaces have very complex layouts and extremely cluttered environments. Also, we want to be able to leverage information about how indoor spaces are designed. While hallways in different office buildings may visually look the same, also with varying sizes (widths) and such, they also do exhibit structural similarities that make it easy to identify what locations in a building are hallways and also what might be connected to it. We leverage this information by categorizing nodes into different classes.

Subsumption architecture

Layers of cognitive map <--> layers of our framework
High level behaviors, low level execution of behaviors vs. topological space reasoning with low level behavior/motor control.

\textit{What we do}

Inspired by studies in psychology, in this work we propose a behavioral navigation topological framework for navigating in indoor environments. Our goal is to perform navigation from one semantic location to another in complex, real-world environments given only a topological map of the space and the current visual input. For example, using a topological map of an office building floor, the agent should be able to navigate from one specific office to another. To do this, we use the Gibson Environment in combination with the Stanford 2D-3D-S dataset for physics-based simulation in realistic settings. The Stanford 2D-3D-S dataset consists of reconstructed meshes of several university buildings, which can have complex layouts and large amounts of clutter (see \textbf{Fig. asdf}).

Two key questions for building such a framework are:
\begin{enumerate}
    \item How to represent the environment
    \item How to plan and execute trajectories in the environment
\end{enumerate}

Our approach is consistent with the subsumption architecture introduced by Brooks. To address (1), we propose a specification for designing topological maps, including what should constitute an node, what should constitute a edge, and how to place the nodes and edges. In our topological map formulation, nodes represent semantic locations such as offices, conference rooms, open spaces, and hallway portions. Similar to Sepulveda et al., we represent each edge as a high-level behavior for getting from one node to another, such as going straight, turning right, or turning left.
% what kind of behaviors should exist

Since the environments have complex layouts and are also filled with clutter, it is easy for the agent to get confused about what action to perform, and also easy for it to collide into objects on the floor. Therefore, to make the system work robustly in such spaces, rather than doing everything jointly, we de-couple our navigation approach into two parts: localization and control.

We structure our navigation approach into two parts: localization and control. At each step, the agent localizes itself within the topological map and then computes and executes the velocity commands based on its current node position and visual input. This cycle of localization and control is repeated until the agent reaches the destination. The decomposition of the action space into primitive behavioral actions is a fundamental component of our approach.

We propose using graph neural networks to localize the agent within the topological map. This is a natural approach for applying deep learning to graphs.

We propose using graph neural networks in combination with convolutional neural networks for localizing the agent in the topological maps

To localize the agent within the topological map, we leverage deep learning and propose using graph neural networks, which is a natural approach when performing computation on graphs. Graph neural networks are particularly suitable for this task because their architecture allows the model to capture the relational inductive biases specified by the topological map. Moreover, feeding the graph as input allows the model to utilize the available affordances help localize itself in the map. For example, we know that we can turn left/right here, so we can't be at that point in the topological map etc etc. Specifically, we first process the visual information using a convolutional neural network (CNN) and pass the visual features along with the topological map to the graph neural network in order to infer the location of the agent. Given a predicted location of the agent within the topological map, it is then simple to compute the path from the current position to the destination, using, for example, a shortest path algorithm.

Once computed, the path translates to a sequence of behaviors (edges in the topological map), including the current behavior to execute. The agent then needs to determine the right controls in order to properly execute the behavior, such as a right turn, and move towards the goal.

In order to robustly execute the behaviors, we propose using a convolutional neural network to translate the visual information into low-level velocity commands for executing the behavior. For example, if the agent is about to exit the office, a neural network trained for turning right can compute the appropriate velocity commands for turning the robot into the hallway. As stated above, this cyclic process of localization and behavior execution is repeated at every timestep until the agent reaches the destination.

We train our models on realistic environments in the Stanford 2D-3D-S using the Gibson simulator. Since we use physics-based simulation, it is essential that our robot does not collide with surrounding objects, furniture, or clutter. Also glass doors, glass walls, and windows.

Using our approach, we show that the agent can successfully navigate in complex, cluttered indoor scenes. By leveraging real-world scenes from the Stanford 2D-3D-S dataset, we are able to use simulation and train our model to be robust to various clutter in the environment. We manually annotated the environment to produce topological maps, which also allowed us to automate some of the data labeling process. Moreover, our approach can generalize to unseen environments and go over long distances and does not rely on explicit visual landmarks. We also provide an evaluation suite.

We need to mention how the topological map is annotated on top of the environment map. This means nodes and edges have specific positions/orientations relative to the /map coordinates, and allows us to automate the annotation process as well as create the evaluation suite.

In summary, our contributions are the following:
\begin{itemize}
    \item We introduce a specification for topological map design in complex, real-world environments.
    \item We propose a novel framework for localization and navigation using convolutional neural networks in conjunction with graph neural networks. By using a behavioral approach, we are able to robustly navigate through realistic environments.
    \item We provide a dataset of video sequences containing RGB, depth, and semantic information along with annotated node localizations, edge behaviors. We also have topological maps which will be released.
    \item We provide a testbed for evaluating navigation tasks using the Gibson Environment along with our topolocial map. The agent can be controlled by running ROS, and our evaluation suite allows us to thoroughly analyze the performance, such the success rates for entering rooms or corridors.
\end{itemize}

==> sec/notes.tex <==
\newpage

\section{Training details (supplemental material)}

Learning rates, optimizer (ADAM), batch size, etc.
Noise injection.
Graph network data augmentation -- should we add an ablation for this? GNN aggregate method.
Architectures can go in appendix.

\section{Previous intro drafts and notes}

Missing:
\begin{itemize}
    \item Extra GT info used by prior work. Simplistic environments. Simplistic physics.
    \item Semantically meaningful action space. Allows behaviors to be trained robustly. Allows actions to generalize to new environments.
    \item What are nodes in the map. How topological maps are connected (what are the edges). What are some example behaviors.
    \item Why graph neural nets.
    \item High level description of the function of each module and the function of the brain. High level description of how the model works.
    \item High level description of graph network module and how it uses context.
    \item Decomposition of action space into primitive but semantically meaningful behaviors.
    \item Cyclic process.
    \item Experiments
    \item Automatic annotation
    \item Eval suite
\end{itemize}
% two components: localization and control. The localization and execution modules are integrated using the Brain.

By using a behavioral navigation approach, we can connect semantic locations in the topological map with edges represented by primitive behaviors that are universal and present in virtually all indoor scenes. For example, behaviors can be turning left, turning right, or even finding a door. Compared to traditional reinforcement learning based approaches, our action space is composed of high-level semantic behaviors, but these behaviors can still be executed robustly and generalized to new environments.

To do this, we use the Gibson Environment in combination with the Stanford 2D-3D-S dataset for physics-based simulation in realistic settings. The Stanford 2D-3D-S dataset consists of reconstructed meshes of several university buildings, which can have complex layouts and large amounts of clutter (see \textbf{Fig. asdf}).

Two key questions for building such a framework are:
\begin{enumerate}
    \item How to represent the environment
    \item How to plan and execute trajectories in the environment
\end{enumerate}

To address (1), we propose a specification for designing topological maps, including what should constitute an node, what should constitute a edge, and how to place the nodes and edges. In our topological map formulation, nodes represent semantic locations such as offices, conference rooms, open spaces, and hallway portions. Similar to Sepulveda et al., we represent each edge as a high-level behavior for getting from one node to another, such as going straight, turning right, or turning left.
what kind of behaviors should exist

Since the environments have complex layouts and are also filled with clutter, it is easy for the agent to get confused about what action to perform, and also easy for it to collide into objects on the floor. Therefore, to make the system work robustly in such spaces, rather than doing everything jointly, we de-couple our navigation approach into two parts: localization and control.

We structure our navigation approach into two parts: localization and control. At each step, the agent localizes itself within the topological map and then computes and executes the velocity commands based on its current node position and visual input. This cycle of localization and control is repeated until the agent reaches the destination. The decomposition of the action space into primitive behavioral actions is a fundamental component of our approach.

We propose using graph neural networks to localize the agent within the topological map. This is a natural approach for applying deep learning to graphs.

We propose using graph neural networks in combination with convolutional neural networks for localizing the agent in the topological maps

To localize the agent within the topological map, we leverage deep learning and propose using graph neural networks, which is a natural approach when performing computation on graphs. Graph neural networks are particularly suitable for this task because their architecture allows the model to capture the relational inductive biases specified by the topological map. Moreover, feeding the graph as input allows the model to utilize the available affordances help localize itself in the map. For example, we know that we can turn left/right here, so we can't be at that point in the topological map etc etc. Specifically, we first process the visual information using a convolutional neural network (CNN) and pass the visual features along with the topological map to the graph neural network in order to infer the location of the agent. Given a predicted location of the agent within the topological map, it is then simple to compute the path from the current position to the destination, using, for example, a shortest path algorithm.

Once computed, the path translates to a sequence of behaviors (edges in the topological map), including the current behavior to execute. The agent then needs to determine the right controls in order to properly execute the behavior, such as a right turn, and move towards the goal.

In order to robustly execute the behaviors, we propose using a convolutional neural network to translate the visual information into low-level velocity commands for executing the behavior. For example, if the agent is about to exit the office, a neural network trained for turning right can compute the appropriate velocity commands for turning the robot into the hallway. As stated above, this cyclic process of localization and behavior execution is repeated at every timestep until the agent reaches the destination.

We train our models on realistic environments in the Stanford 2D-3D-S using the Gibson simulator. Since we use physics-based simulation, it is essential that our robot does not collide with surrounding objects, furniture, or clutter. Also glass doors, glass walls, and windows.

Using our approach, we show that the agent can successfully navigate in complex, cluttered indoor scenes. By leveraging real-world scenes from the Stanford 2D-3D-S dataset, we are able to use simulation and train our model to be robust to various clutter in the environment. We manually annotated the environment to produce topological maps, which also allowed us to automate some of the data labeling process. Moreover, our approach can generalize to unseen environments and go over long distances and does not rely on explicit visual landmarks. We also provide an evaluation suite.

We need to mention how the topological map is annotated on top of the environment map. This means nodes and edges have specific positions/orientations relative to the /map coordinates, and allows us to automate the annotation process as well as create the evaluation suite.

\section{Consider: Description of Areas}

For example, what is the difference between area 3 and 4. Given there's such a large performance gap...it's actually not because one is val set and one is test set. It's because the val set looks similar to the train set, and is also a lot smaller area.

We probably need to spend a day on the video. It is crucial to make a good video.

We crop the graph by the removing nodes/edges that are more than 3rd order neighbors or higher.

% \subsection{Realism}

\begin{itemize}
    \item Collisions (House3D, SPTM, Gupta, Sepulveda, etc.)
    \item Provided GT egomotion (Mirowski, Gupta, Parisotto)
    \item Realistic environments (house3d, suncg, ai2thor count as realistic environments). works that don't: sptm, sepulveda, mirowski
    \item physics based / continuous action space: has anybody done this? works that don't: gupta, sptm, sepulveda, mirowski, yang (visual sem nav using scene priors), house3d
\end{itemize}

Physics
Collisions are basically guaranteed failures, unlike works like House3D, etc. Especially because the robot can't move in arbitrary directions, whereas they can in many synthetic settings (e.g. House3D).

Environment clutter, etc. etc.

Add a key for sample plan images for how long 1 meter is relative to the rest of the map.

Add an example of navigation trajectories shown in Gupta? For reference...ours are way longer.

\section{Useful info for intro}

Key questions regarding cognitive maps:
How to design a topological map
Nodes are places or visual landmarks, but still, what should be a node?
How do we connect the landmarks? What is the right representation to use?

\textbf{Motivation and stuff from prior works}

Successful navigation is not dependent on geometric accuracy, since the control and topology
levels do not depend on the geometric description . However, when geometric information is
available, it can be used to optimize route-planning or to resolve topological ambiguities .

``Many scientists [29,35,39] have observed that a
cognitive map is organized into successive layers,
and suggested that the central element of a useful
and powerful description of the large-scale environment is a topological description . A layered
model consists of the identification and recognition of landmarks and places from local sensory
information ; control knowledge of routes (procedures for getting from one place to another) ; a
topological model of connectivity, order, and containment ; and metrical descriptions of shape, distance, direction, orientation, and local and global
coordinate systems . It appears that the layered
structure of the cognitive map is responsible for
humans' robust performance in large-scale space .
Our approach attempts to apply these methods to
the problem of robot exploration and map-learning.'' from Kuipers

 Laumond [26] and
Chatila and Laumond [6] build a topological model
from the geometric model and then derive a
semantic model, e .g . identifying 'rooms' and `corridors', from the topological model . Their approach uses the topological description to represent map information at higher levels of abstraction . However, there is no use of the topological
model to cope with metrical inaccuracy .

Gupta:
More crucially, classical approaches rely entirely on observed evidence and do not use priors and experience from similar other environments to
make meaningful inferences about unobserved parts of the
environment

Contemporary learning based approaches [23, 37] have
focused on incorporating such statistical priors, but have
largely ignored the question of representation of spaces by
making it completely implicit in the form of neural network activations. Works that do build spatial representations (such as [12]), operate under ideal world assumptions
where the agent is always aware of its exact location in the
environment.

 even rats build sophisticated representations for space in the form of ‘cognitive maps’ as they navigate, giving them the ability to reason
about shortcuts, something that a reactive agent is unable to

It is at this point that humans are
also able to plan paths to novel places and find shortcuts
for going between different known points. This is generally
accomplished by reasoning over a coarse spatial layout of
places through a cognitive map [33].

Bajcsy et al:
On the other hand, research by cognitive psychologists (Kozlowski and
Bryant [15], Shepard [37], Pylyshyn [33]) and zoologists (Schone [36]) has
clearly demonstrated that humans and animals record distinctive visual landmarks and use the structure inherent in local and temporal relationships
between landmarks relative to observer paths of motion, in order to predict
and identify places in the world and to plan and execute paths between
locations

Semi parametric topo map:
However, extensive evidence from psychology suggests that when traversing environments, animals do not rely strongly on metric representations (Gillner and Mallot, 1998; Wang and Spelke, 2002; Foo et al., 2005). Rather, animals employ a range of specialized navigation strategies of increasing complexity. According to Foo et al. (2005), one such strategy is landmark navigation – “the ability to orient with respect to a known object”. Another is route-based navigation that “involves remembering specific sequences of positions”. Finally, map-based navigation assumes a “survey knowledge of the environmental layout”, but the map need not be metric and in fact it is typically not: “[. . .] humans do not integrate experience on specific routes into a metric cognitive map for navigation [. . .]. Rather, they primarily depend on a landmark-based navigation strategy, which can be supported by
qualitative topological knowledge of the environment.”

\textbf{Outline}:
\begin{itemize}
  \item Motivation
  \item Prior works
  \item Summary of our approach
\end{itemize}

\textbf{Goal}: Navigate from A to B in both seen and unseen environments using topological maps
\begin{itemize}
    \item No metric information
    \item No explicit visual landmarks
    \item Long-distance navigation goals
    \item Real-world environments
\end{itemize}

\textbf{Contributions}:
\begin{itemize}
    \item First to use graph nets for localization in topological maps and plan execution
    \item Method for executing behaviors robustly (without crashing)
    \item Handle real-world environments (full of clutter and uses complex maps)
    \item Design set/rules of topo map
    \item Topological map annotations in real-world dataset (with mesh)
    \item Create a new testbed for evaluating navigation tasks, and provide an evaluation suite
\end{itemize}

Useful references when writing intro
\begin{itemize}
    \item Cognitive mapping, unifying landmarks, etc.
    \item Vladlen semi-parametric topological maps
\end{itemize}

Make sure to discuss the following:
\begin{itemize}
  \item How humans navigate (e.g. human vs rat navigation paper)
  \item Robustness to changing state of same environment (clutter that moves around, rearranging of furniture, complete remodel of environment like in 1st floor AI lab).
  \item Most research in DRL focuses on simplistic, synthetic environments
  \item Reliance on accurate metric information makes methods brittle
  \item EMNLP submission
\end{itemize}

==> sec/related-v1.tex <==
\begin{figure}
    \begin{subfigure}{0.35\linewidth}
    \includegraphics[width=\linewidth]{fig/topological_map_input_office.pdf}
    \caption{Entering a room}
    \label{fig:toy-topological-map-room-enter}
    \end{subfigure}
    \rulesep
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[width=\linewidth]{fig/topological_map_out_of_office.pdf}
    \caption{Exiting a room}
    \label{fig:toy-topological-map-room-exit}
    \end{subfigure}
    \rulesep
    \begin{subfigure}{0.25\linewidth}
    \includegraphics[width=\linewidth]{fig/topological_map_intersection.pdf}
    \caption{Entering an intersection}
    \label{fig:toy-topological-map-intersection}
    \end{subfigure}
    \caption{Examples of the topological map cropped to the local region of the agent.}
    \label{fig:toy-topological-map}
\end{figure}

\section{Related Work}

There is a long history of prior work on robot localization and navigation within mobile robotics. Due to limited space, we do not provide a comprehensive review but refer interested readers to \cite{Filliat03:article, thrun2005probabilistic, siegwart2011introduction} for a broader overview of related work. The following paragraphs focus on describing close and, especially, recent efforts related to our work.

While dominant approaches for robot navigation rely on fine-grained geometric representations of the world, alternative deep learning approaches have recently gained interest due to limitations of classical methods in terms of generality and robustness. The deep learning approaches may be reactive \cite{zhu2017target,dosovitskiy2016learning} or utilize memory. For example, memory can be implemented through general-purpose neural network modules, like Long Short-Term Memory networks (LSTM) \cite{mnih2016asynchronous,mirowski2016learning}, or based on a metric map \cite{gupta2017cognitive,gupta2017unifying}. % For example, \citet{gupta2017cognitive, gupta2017unifying} propose architectures inspired by theories of spatial cognitive maps \cite{tolman1948cognitive, trullier1997biologically}.
Recently, \citet{savinov2018semi} introduced a deep learning-based method for navigating using topological representations. Different to our task, though, their problem setup assumes that the agent has already explored the navigation environment to collect  visually encoded waypoints. % Likewise, \citet{mirowski2016learning, brahmbhatt2017deepnav} focus on end-to-end, task-driven models for navigation. 

Our particular approach to robot navigation builds on a recent effort by Sepulveda et al. \cite{sepulveda2018deep} on enabling indoor navigation with deep visuo-motor behaviors \cite{pomerleau1989alvinn, muller2006off, bojarski2016end}. Their prior work is inspired by early efforts on behavioral robotics \cite{brooks1986robust, horswill1993polly} and topological navigation \cite{kuipers1991robot}. Similar to \cite{sepulveda2018deep}, our aim is to take full advantage of the rich semantic structure behind man-made environments for navigation, and leverage simple robot behaviors to complete complex tasks. We avoid reliance on metric information \cite{parisotto2017neural}, robot odometry \cite{gupta2017cognitive}, or specific poses that need to be attained during indoor navigation \cite{gupta2017unifying}. But different to \cite{sepulveda2018deep}, we depart from a large repertoire of behaviors for the problem of indoor navigation. This change was needed to (1) facilitate the design of topological maps for realistic, human environments, and (2) increase the robustness of learned navigation behaviors given limited data. Additionally, our approach does not need artificial landmarks, as in \cite{sepulveda2018deep}, to enable a robot to sequentially execute navigation behaviors towards a desired goal location. 

There is a connection between our work and prior efforts on compositionality \cite{andreas2017modular,andreas2016neural} and learning sequencing of manipulation primitives \cite{felip2013:article}. The connection stems from navigation behaviors and primitives  conceptualizing atomic actions executable by a robot. These actions aim to reduce the dimensionality of movement control \cite{mataric1998behavior, kallmann2004planning}. However, different to recent work on robot manipulation \cite{ntp18:inproceedings, huang2018neural, yu2018one}, our goal is not to figure out how to solve new tasks given demonstrations of an ordered set of actions. Instead, our goal is to execute an abstract navigation plan given a topological map of a realistic, and often cluttered, human environment. 
%In our case, the plan corresponds to a path in the map. Both the plan and the map are given in our problem setting. 

A key component of our navigation approach is a localization network that leverages graph neural networks \cite{scarselli2009graph,battaglia2018relational}. While other related efforts have used similar kinds of neural networks for navigation, e.g.,  \cite{yang2018visual} uses graph convolutional networks \cite{kipf2016semi} to encode semantic priors; we are the first to use these networks to estimate coarse location with respect to a topological map to the best of our knowledge.

We test our proposed approach with Gibson, an embodied environment for real-world perception \cite{xiazamirhe2018gibsonenv} of large-scale indoor spaces \cite{armeni_arxiv_2d3ds}. In particular, we create topological maps for the latter indoor spaces and extend the capabilities of Gibson in order to create a benchmark for behavioral robot navigation. With this effort, we join others, e.g., \cite{wu2018building, Dosovitskiy17}, in building a rich and extensible environment for mobile robotics and machine learning research. We hope to encourage the community to move away from evaluations in more artificial environments \cite{mirowski2016learning, savinov2018semi, sepulveda2018deep}. 
% More details about this contribution are provided in Sec. \ref{}.

 


% Related work.

% Here are some related works to cite:
% \begin{itemize}
%     \item Cognitive Mapping and Planning for Visual Navigation: They use the idea of cognitive mapping but use GT egomotion. The shown navigation plans look very short. They use a navigation memory structure based on a metric map. It looks like collisions are allowed, but hard to confirm.
%     \item Unifying Map and Landmark Based Representations for Visual Navigation. Similar to the previous work...they want to avoid complete reliance on classical/geometric approaches.
%     \item Neural map: Memory structure based on metric map
%     \item Semi-parametric Topological Memory for Navigation: This one is pretty cool. They build a topological map of the environment as they navigate. They use fake environments though (Doom I think). Also it looks like collisions are allowed based on the videos.
%     \item A Deep Learning Based Behavioral Approach to Indoor Autonomous Navigation. Similar to our work. You guys know this. Also, collisions are allowed.
%     \item Learning to Navigate in Complex Environments: These guys use pretty synthetic/fake environments and ground truth ego-motion. They use unstructured general-purpose memory like LSTM
%     \item Visual Semantic Navigation Using Scene Priors: AI2 thor. They use a graph to encode priors about where objects may be located, and use a graph convolutional network.
%     \item Building generalizable agents with a realistic and rich 3D environment: Collisions are allowed I think.
%     \item Yuke Zhu and Alexey Dosovitskiy's early papers on DL-based approaches for navigation using reactive models.
%     \item One-Shot Hierarchical Imitation Learning of Compound Visuomotor Tasks: Compounding primitive actions
%     \item Graph neural networks and its variants like Kipf and Welling, etc.
%     \item Other prior work on behavioral navigation
%     \item Hierarchical RL
% \end{itemize}
